The Success of AdaBoost and Its Application in Portfolio Management

We develop a novel approach to explain why AdaBoost is a successful classifier. By introducing a measure of the influence of the noise points (ION) in the training data for the binary classification problem, we prove that there is a strong connection between the ION and the test error. We further identify that the ION of AdaBoost decreases as the iteration number or the complexity of the base learners increases. We confirm that it is impossible to obtain a consistent classifier without deep trees as the base learners of AdaBoost in some complicated situations. We apply AdaBoost in portfolio management via empirical studies in the Chinese market, which corroborates our theoretical propositions.

==> secs/iintro_backup.tex <==
\section{Introduction}

% Previous work and literature.

% \subsection{Background}
Equal-weighted long-short portfolios are one of the most important strategies in stock investment management of hedge funds. 
In general, it is a portfolio whose weights are equally distributed across the selected securities separately in the long and short positions.
It is different from the mean-variance optimized portfolio of \citet{markowitz1952}.

% The portfolios are important in finance.
In the asset pricing area, \citet{famafrench1993, famafrench2015} construct the equal-weighted long-short portfolios as the factor proxies of SMB (the size) and HML (the value);
\citet{feng2017zoo} tested the validation of 150 factors, and many of them are generated by the long-short portfolios.
In portfolio optimization,
numerous studies have suggested that equal-weighted long-short portfolios outperform other portfolios when tested in an out-of-sample context (e.g., \citealt{jobson1981}; \citealt{james2003bias_variance}).
\citet{michaud1989markowitz} and \citet{demiguel2007_1n} argued that it is because they do not suffer from the estimation error of the covariance matrix, which is vulnerable to extreme values \citep{tu2011}.
\cite{allen2019_Portfolio} also showed that equal-weighted long-short portfolios outperform when the forecast ability is low.
In industry, equal-weighted long-short portfolios are popular in hedge funds.
MSCI has issued many equal-weighted indexes, which, it said, are ``some of the oldest and best-known factor strategies that have aimed to identify specific characteristics of stocks generating excess return''.

The core of the equal-weighted long-short strategy is to forecast long and short positions, a classification problem of factor model; 
Machine learning achieves highly in classification problems, thus effectively dealing with the equal-weighted long-short portfolios. 
The research of machine learning on classification is hugely diverse. 
The monograph, \citet{DGL1996}, lists numerous  traditional pattern recognition research in computer science, where pattern recognition is another name of the classification problem. 
Another masterpiece, \citet{book:esl}, analyzes and summaries many machine learning methods, in which classification methods are the Linear/Quadratic Discriminant Analysis, Support Vector Machine, Boosting, Random Forest, and so on. 
The application of machine learning in classification succeeds in various fields, such as email spam, handwritten digit recognition, etc.
In portfolio management, the monograph \citet{de2018ml} explained how to apply machine learning to manageing funds for some of the most demanding institutional investors.
Specifically,
\citet{creamer2005AdaBoost, creamer2010automated} applied the Boosting method in finance, revealing its practical value.
\citet{creamer2012model} used LogitBoost in high-frequency data for Euro futures, generating positive returns.  
\citet{wang2012DB} invented the N-LASR (non-linear adaptive style rotation) model by applying AdaBoost in factor models.
Its organically incorporated factors benefit the N-LASR model with interpretation and significant empirical risk-adjusted return on the component stock in Russel  3000.
\citet{fievet2018trees} proposed a decision tree forecasting model, capable of capturing arbitrary interaction patterns and generating positive returns.
\citet{rasekhschaffe2019_ML_stock_selection} provided an example of the machine learning techniques to forecast the cross-section of stock returns.
\citet{gu2018_ML_asset_pricing} and \citet{dhondt2020} gave a comprehensive analysis of machine learning methods for the canonical problem of empirical asset pricing, attributing their predicted gains to the non-linearity.


AdaBoost is a classification method in machine learning, inspiring a tremendous amount of innovations. 
AdaBoost has developed for more than two decades. 
\citet{freund1996adaboost} brought about AdaBoost, answering the questions raised by \citet{kearns1989}. 
Because it is hard to overfitting, Breiman praised AdaBoost---``the best off-the-shelf classifier in the world''---at the 1996 NeurIPS conference \citep{friedman2000additive}.
AdaBoost has made a significant impact on machine learning and statistics. 
To explain the anomaly, \citet{schapire1998boosting} argued that the margin results in the overfitting resistance property.
Meanwhile, \citet{breiman1998arcing, breiman1999prediction, friedman2000additive} discovered the fact that AdaBoost is equivalent to an optimization algorithm, so \citet{friedman2001greedy} brought about the Gradient Boosting. 
Inspired by AdaBoost, \citet{breiman2001random} invented the Random Forest and believed that there is some similarity between it and AdaBoost. 
Subsequently, people generalized the Boosting methods, in which two Boosting algorithms are widely-adopted, XGBoost \citep{XGBoost} and LightGBM \citep{LGBM}. 
Till now, the family of Boosting flourishes, taking up a considerable part in machine learning. 

As the AdaBoost development,
there is much literature explaining why AdaBoost is a successful classifier.
For instance, 
\citet{schapire1998boosting} attributed the success of AdaBoost to the margin, 
and \citet{friedman2000additive} regarded it as an optimization problem.
Till now, people are still curious about its success.
\citet{wyner2003OnBA} and \citet{mease2008contrary} believed that the available interpretation of AdaBoost is ``incomplete'', particularly on the explanation of the overfitting resistance property.  
\citet{wyner2017AdaBoost_RandomForest} introduced a novel perspective on AdaBoost and conjectured that AdaBoost's succeed could be explained by the concept of ``spiked smooth'', a self-averaging interpolating algorithm.
In other words, the algorithm is localizing the effect of the noise points in a ``spiked smooth'' method.
Based on this idea, we believe that this property may have outstanding performance in low signal-to-noise ratio situations.

% \subsection{Motivation}

Our work is motivated by the industry's questions: 
``May machine learning outperforms in quantitative investment? Why? How it works.''
\citet{de2018ml} gave a comprehensive and systematic approach to apply machine learning methods,
in which he highly appraised Boosting:
``We explored a number of standard black-box approaches. Among machine learning methods, we found gradient tree boosting to be more effective than others.'' \citep[p. 341]{de2018ml}.
Besides, \citet{zhang2019boosting} proposed a Boosting method to compose portfolios and performed well.
 \cite{wang2012DB}
applied AdaBoost to select and combine factors with consistent and interpretable outperformance.
These findings answered the first question.
% and did not explain why and how AdaBoost performs well.
There is little research concerning the mechanism or the interpretability of machine learning in investment.
However,
explainability is essential in investment \citep{feng2017zoo}. 
In detail, 
\citet[p. 37]{harvey2016and} argued:
``[...] a factor developed from first [economic] principles should have a lower threshold t-statistic than a factor that is discovered as a purely empirical exercise.''
\citet{harvey2017presidential} formed portfolios based on the first, second, and third letters of the ticker symbol, gaining significant excess returns.
Nevertheless, nobody would adopt this symbolic portfolio at all.
Thus, without explainability, portfolio investment is vulnerable.
People need to answer the second/third questions.

Inspired by \citet{wyner2017AdaBoost_RandomForest}, we investigate AdaBoost in the framework of statistics to find a theoretical explanation of its outperformance and apply them in portfolio investment.
They pointed out that:
``The statistics community was especially confounded by two properties of AdaBoost: 1) interpolation (perfect prediction in sample) was achieved after relatively few iterations, 2) generalization error continues to drop even after interpolation is achieved and maintained.''
They innovated the ``spiked smooth'' classifier created by a self-averaging, interpolating algorithm.
They conjectured that it renders AdaBoost successful by simulation. 
They provided many delicate examples to support their explanation.
Thus, we would like to narrow the gap between the theory and simulation by strengthening their work from a statistical perspective. 
To explain the ``spiked smooth'' from a mathematical perspective, we need to define signal and noise in a statistical framework first.
Furthermore, we translate their interpolation definition into our statistical framework.
Then, one should connect the relationship between the ``spiked smooth'' and the test error, 
so she could apply the ``spiked smooth'' to explain the property of overfitting resistance.

In addition, \citet{wyner2017AdaBoost_RandomForest} also pointed out that  ``boosting should be used like random forests: with large decision trees, without regularization or early stopping''. 
That is to say, larger and deeper decision trees are preferred to be used as the weak classifiers of AdaBoost since they can ``interpolate'' the samples and realize the goal of ``spiked-smooth''. 
This concept is contradicted with common sense about machine learning and statistics since statisticians usually believe complexity leads to overfitting. 
Therefore, inspired by \citet{wyner2017AdaBoost_RandomForest}, we wonder if the AdaBoost algorithm can boost weak classifiers once the weak ones are too weak, just as we cannot ``make bricks without straw''. We try to find out that under what populations will the AdaBoost algorithm cannot achieve good performance if the weak classifiers are very weak. We want to demonstrate the viewpoints of \citet{wyner2017AdaBoost_RandomForest} more mathematically. 


% \citet{wyner2017AdaBoost_RandomForest}关于``spiked smooth''的概念很新颖也有数值计算的验证, 但却缺乏统计模型的理论基础。
% 要从统计推断的基本框架来定义signal和noise, 并进而对``spiked smooth"的概念给出定义。还要建立``spiked smooth"与
% generalized error 关系, 从本质上解释 the overfitting resistance property.

% \subsection{Our Work}

In this paper, 
we specify the questions into a detailed investment portfolio construction. 
We strict the research in the fields of equal-weighted portfolios. 
Consequently, we can utilize the theory of classification problems to develop further analysis.
% We argued that,
% when signal-to-noise ratio is low,
% classification problems are more powerful. 
We focus on AdaBoost in detail, which is one of the most influential machine learning algorithm.
We argued that AdaBoost can dig out more non-linear information with little impact from over-fitting or noise.

Our work is composed of three parts.
First, 
We interpret that AdaBoost ``with large decision trees without [...] early stopping is better'',
showing its overfitting resistance with respect to noise.
In detail,
we define a measure for the influence of the noise points in a training set, which concretes the abstract concept ``spiked-smooth''.
We prove its connection with the out of sample performance of machine learning methods;
That is, under a certain condition, if the influence of the noise point is low, then the test error is low.
For AdaBoost, we further collaborate the conjecture of \citet{wyner2017AdaBoost_RandomForest}, showing that, 
as the iteration number or the depth of the base classifier grows, the ION of AdaBoost decreases, 
and so is the test error.
Thus, 
we explains why a certain kind of AdaBoost outperforms.

Second, we confirm that it is a better choice to use deeper/larger decision trees as weak classifiers in AdaBoost in the sense of digging out complex information. 
Specifically,
We propose several counter examples that AdaBoost with shallow decision trees fails to handle, no matter how high the iteration number is.
We generalize the results to particular properties, indicating that AdaBoost based on shallow decision trees would only recognize a certain kind of information, while AdaBoost with deep decision trees could easily solve out.
Therefore, these findings suggest AdaBoost with deep decision trees may be better.

Third, empirical study in Chinese market collaborate our theoretical proposition.
SOMEONE ADDS MORE WORDS.

The outline of this paper is as follows.
Section~\ref{sec:ION and AdaBoost} explains why AdaBoost succeeds by defining a measure.
Section~\ref{sec:XOR_counter} shows that AdaBoost with deep trees can dig out more information.
Section~\ref{sec:empirical} is the empirical study of AdaBoost in Chinese stock market.
Section~\ref{sec:conclusion} concludes.



==> secs/proofs.tex <==
% \section{Appendix: proofs}

==> secs/temp.tex <==
\iffalse
\section{Basic concept of AdaBoost}


\subsection{The training error and test error}

\begin{defn}
Given the population of $(X, Y)$ and the sample $T=(\bm{x}_i, y_i)_{i=1}^n$,
for a classifier $f$ trained on $T$,
the training error is defined as
\begin{align}
    \text{Training error} :=
    \frac{1}{n}\sum_{i=1}^n \mathbbm{1}\{f(\bm{x}_i)\neq y_i\},
\end{align}
and the test error is defined as
\begin{align}
    \text{Test error} :=
    \mathbb{P}\{f(X)\neq Y\}.
\end{align}
The test error is also called the generalization error.
\end{defn}



\subsection{The algorithm of AdaBoost}

There are various versions of AdaBoost.
Consistent with \citet{wyner2017AdaBoost_RandomForest}, 
we list the almost original algorithm of AdaBoost.M1 in \citet{book:esl} as Algorithm~\ref{alg:adaboost}.
\begin{algorithm}
	\caption{AdaBoost.M1 \citep{book:esl}\label{alg:adaboost}}
	\begin{enumerate}
		\item[0.] Given the sample $ T = (\bm{x}_{i}, y_{i})_{i=1}^{n} $, where $ y_{i} \in \{\pm 1\} $. Determine exogenous parameters of maximum iteration $ M $, and the maximum depth of the base learners (such as CART, \citet{breiman1984CART}).
		\item Initialize the weights $ \omega^{1}_{i} = \frac{1}{n}, i = 1, 2, 3, \cdots, n.$
		\item For $ m = 1, 2, 3, \cdots, M $:
		\begin{enumerate}
			\item Fit a classifier $ g^{m}(\bm{x}) $ to the sample using weights $ {\omega}^{m} $: $ (\bm{x}_{i}, y_{i}; \omega_{i}^{m})_{i=1}^{n} $.
			\item Compute the error with weights
			\[
			\mathrm{err}^{m} = \frac{\sum_{i=1}^{n} \omega_{i}^{m} \mathbbm{1}\{y_{i}\neq g^{m}(\bm{x}_{i})\}}{\sum_{i=1}^{n} \omega_{i}^{m}}.
			\]
			\item Compute the log odds with weights
			\[
			\alpha^{m} = \log \frac{1-\mathrm{err}^{m}}{\mathrm{err}^{m}}.
			\]
			\item Update weights
			\[
			\omega_{i}^{m+1} = \omega_{i}^{m} \cdot \exp\left(\bigg.
			\alpha^{m} \cdot \mathbbm{1}\{y_{i}\neq g^{m}(\bm{x}_{i})\}
			\right), i = 1, 2, 3, \cdots, n.
			\]
		\end{enumerate}
		\item Output $ \mathrm{sign}\{f^{M}(\cdot)\} $, where $ f^{M} =  \sum_{m=1}^{M} \alpha^{m}  g^{m}. $
	\end{enumerate}	
\end{algorithm}

\subsubsection{Decomposition}
\begin{align}
\mathbb{P}_X\{f_T(X) \neq f^B(X)\}
=&\ 
\mathbb{P}_X\{f_T(X) \neq f^B(X), f_T(X) \neq f_{T_p}(X)\}
+
\mathbb{P}_X\{f_T(X) \neq f^B(X), f_T(X) = f_{T_p}(X)\}
\end{align}

$\mathbb{P}_X\{f_T(X) \neq f^B(X), f_T(X) \neq f_{T_p}(X)\}$ represents the influence of the noise on the sample $T$, 
which is implied in $y|X$.
In contrast, 
$\mathbb{P}_X\{f_T(X) \neq f^B(X), f_T(X) = f_{T_p}(X)\}$ is the influence of the information $\bm{x}_i$ of the sample points $(\bm{x}_i, y_i)$, 
which is implied only in $X$.
In short,
the former one is about the noise,
the latter one is about the luck, i.e., the sample distribution of $X$.

\fi
